Deriving Generic Bounds for Time-Series Constraints Based on Regular Expressions Characteristics

We introduce the concept of regular expression characteristics as a unified way to concisely express bounds on time-series constraints. This allows us not only to define time-series constraints in a compositional way, but also to deal with their combinatorial aspect in a compositional way, without developing ad-hoc bounds for each time-series constraint separately.

==> benchmark.tex <==
\section{Benchmark}
\label{sec:bench}

% Do NOT erase the following lines:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "bounds.tex"
%%% End:

==> computing-range.tex <==
\subsection{Simplifying Computation of Range In Some Cases}
\todotext{Cette section peut \^etre enlev\'ee!}
\label{sec:simpl-range}
It may be hard to compute the range of a reglar expression in the
general case.
%
We define properties of regular expressions that allow us easily
obtain the range of a given regular expression~$\pattern$ that
satisfies  Condition~\ref{Cond:a}, and of the two
Conditions~\ref{Cond:b} or~\ref{Cond:c}:

\setword{(a)}{Cond:a}~There exists a shortest word
in~$\Language{\pattern}$ whose height equals~$\Char{\Height}{\pattern}$.

\setword{(b)}{Cond:b}~$\pattern$ is a disjunction-capsuled regular expression.

\setword{(c)}{Cond:c}~$\pattern$ is a disjunction of disjunction-capsuled regular
expressions~$\pattern_1$ and~$\pattern_2$ that are mirrors.

It can be shown that two regular expressions that are mirrors have the
same value of range for any time-series length~$\seqlength$.
%
We denote by~$\pattern^*$ the regular expression~$\pattern$ itself if
it satisfies Condition~\ref{Cond:b} and~$\pattern_1$ if~$\pattern$ satisfies
Condition~\ref{Cond:c}.
%
The regular expression~$\pattern^*$ is disjunction-capsuled and has the
single inducing words, whose height equals~$\Char{\Height}{\pattern}$.
%
Further, we present four properties on the structure of~$\pattern^*$,
which allow us obtain the value of~$\CharPar{\Range}{\pattern}{\seqlength}$:

\begin{enumerate}
\item 
  $\UnconditionalEquality$:
  a regular expression~$\pattern^*$ is of the form either ~$\reg{r_1=^*r_2}$
  or~$\reg{r_1(=| r_2 | \dots |  r_m)^*r_{m+1}}$, where $r_1,\dots,r_m$ are
  disjunction-capsuled regular expressions, possibly, empty.
  % 
  This is the case, when the inducing word~$\wordu$
  of~$\Language{\pattern^*}$ can be
  extended by inserting an arbitrary number of equalities.
  % 
  Hence, for any time-series length~$\seqlength > |\wordu| + 1$, we
  have~$\CharPar{\Range}{\pattern}{\seqlength}$ being~$\Char{\Height}{\pattern}$ and
  $\Tuple{\Char{\FullExtFreeCoeff}{\pattern}, \Char{\FullExtLinCoeff}{\pattern}}$
  being $\Tuple{0,0}$.
  
\item 
  $\Pereodicity$:
  a regular expression~$\pattern^*$ is of the form either~$\reg{(ab)^*(a |
    \varepsilon)}$, where~$a \neq \reg{=}$,~$b \neq \reg{=}$ are mirror
  letters of the alphabet~$\Sigma$.
  % 
  This is the case when every word of~$\Language{\pattern^*}$ of even
  length is periodic with the period of two and every word of odd
  length has a periodic prefix with the period of two and a suffix of
  length~$1$.
  %
  Since~$a$ and~$b$ are mirrors, the words $\reg{(ab)^2}$ and~$\reg{aba}$ have the
  same total shift as~$\reg{ab}$, which is the inducing word of~$\pattern^*$.
  %
  Hence, for any time-series length~$\seqlength > |\wordu| + 1$, we
  have~$\CharPar{\Range}{\pattern}{\seqlength}$ being~$\Char{\Height}{\pattern}$ and
  $\Tuple{\Char{\FullExtFreeCoeff}{\pattern}, \Char{\FullExtLinCoeff}{\pattern}}$
  being $\Tuple{0, 0}$.

\item 
  $\ConditionalEquality$:
  a regular expression~$\pattern^*$ is of the form either~$\reg{r_1(a=^*)^*r_2}$, 
  or~$\reg{r_1(a_1(= | a_2 | \dots | a_t)^*)^*r_2}$,
  where $r_1, r_2$ are disjunction-capsuled regular expressions, $a,
  a_1, \dots a_t$ are letters of the alphabet~$\Alphabet$, and the
  height of the word $\reg{r_1a}$ equals the height of~$r_2$ plus
  one.
  %
  This is the case, when the minimal difference of the heights of a shortest word and of any
  longer word is at 1.
  %
  Hence, for any time-series length~$\seqlength > |\wordu| + 1$, we
  have~$\Char{\Range}{\pattern}{\seqlength}$ being~$1$ and
  $\Tuple{\Char{\FullExtFreeCoeff}{\pattern}, \Char{\FullExtLinCoeff}{\pattern}}$
  being $\Tuple{0, 1}$.

\item 
  $\NoEquality$:
  a regular expression is of the form~$\reg{a^+}$, where $a \neq
  \reg{=}$ is a letter of the alphabet~$\Alphabet$.
  % 
  This is the case when no word of~$\Language{\pattern}$ contains
  equality symbols.
  %
  Hence, for any time-series length~$\seqlength > |\wordu|+1$, we
  have~$\CharPar{\Range}{\pattern}{\seqlength}$ being~$\seqlength - 1$ and
  $\Tuple{\Char{\FullExtLinCoeff}{\pattern},
     \Char{\FullExtFreeCoeff}{\pattern} }$ being~$\Tuple{1,0}$.
\end{enumerate}

Every regular expression in~\tabref{tab:patterns} has at least one of
the four properties listed above, its range can be computed easily.

\begin{example}
  \label{ex:simpl-range}
  Consider
  a~$\Constraint{max\_width}\_\pattern(\XSeq,
  \Result)$ time-series constraint with every~$X_i$ ranging over the same integer interval
  domain~$\Domain$.
  % 
  We consider three different values of~$\pattern$ and compute the sharp
  upper bound on the value of~$\Result$ in the three cases.

  \begin{itemize}

  \item
    Let~$\pattern$ be the~$\InflexionPatternName =
    \InflexionPattern$ regular expression.
    %
    The word, say~$\reg{<>}$, is a shortest word
    in~$\Language{\pattern}$ and its height
    equals~$\Char{\Height}{\pattern}$, namely~$1$.
    %
    Hence,~$\pattern$ satisfies~\condref{Cond:a}.
    %
    Furthermore,~$\pattern$ can viewed as~$\pattern_1 | \pattern_2$, where
    both~$\pattern_1$ and~$\pattern_2$ are disjunction-capsuled
    regular expressions and mirrors, thus~$\pattern$ satisfies~\condref{Cond:c}. 
    %
    Then,~$\pattern_1$ is of the form~$\reg{<(<|=)^*>}$,
    thus~$\pattern$ has~$\UnconditionalEquality$ property.

  \item
    Let~$\pattern$ be the~$\ZigzagPatternName =
    \ZigzagPattern$ regular expression.
    %
    The word~$\reg{><>}$, is a shortest word
    in~$\Language{\pattern}$ and its height
    equals~$\Char{\Height}{\pattern}$, namely~$1$.
    %
    Hence,~$\pattern$ satisfies~\condref{Cond:a}.
    %
    Furthermore,~$\pattern$ can viewed as~$\pattern_1 | \pattern_2$, where
    both~$\pattern_1$ and~$\pattern_2$ are disjunction-capsuled
    regular expressions and mirrors, thus~$\pattern$ satisfies~\condref{Cond:c}. 
    %
    Then,~$\pattern_1$ is of the form~$\reg{(ab)^*(a | \varepsilon)}$,
    where~$a$ is~$<$ and~$b$ is~$>$, thus~$\pattern$
    has~$\Pereodicity$ property.
    
  \item
     Let~$\pattern$ be the~$\GorgePatternName =
    \GorgePattern$ regular expression.
    %
    The word~$\reg{><}$, is a shortest word
    in~$\Language{\pattern}$ and its height
    equals~$\Char{\Height}{\pattern}$, namely~$1$.
    %
    Hence,~$\pattern$ satisfies~\condref{Cond:a}.
    %
    Furthermore,~$\pattern$ is a disjunction-capsuled
    regular expression, thus~$\pattern$ satisfies~\condref{Cond:b}. 
    %
    Finally, any word longer than~$\Char{\width}{\pattern}$
    in~$\Language{\pattern}$ has a height of at
    least~$\Char{\Height}{\pattern} + 1$, thus~$\pattern$
    has~$\ConditionalEquality$ property.   

  \item
    Let~$\pattern$ be the~$\StrictlyDecreasingSequencePatternName =
    \StrictlyDecreasingSequencePattern$ regular expression.
    %
    The word~$\reg{>}$, is a shortest word
    in~$\Language{\pattern}$ and its height
    equals~$\Char{\Height}{\pattern}$, namely~$1$.
    %
    Hence,~$\pattern$ satisfies~\condref{Cond:a}.
    %
    Furthermore,~$\pattern$ is a disjunction-capsuled
    regular expression, thus~$\pattern$ satisfies~\condref{Cond:b}. 
    %
    Finally,~$\pattern$ is of the form~$a^+$, where~$a$ is~$\reg{<}$, 
    thus~$\pattern$ has~$\NoEquality$ property.   \qed
    
    \end{itemize} 
  \end{example}

==> context.tex <==
\section{Context}
\label{sec:context}

Consider a time-series constraints $\Constraint{g\_f}\_\pattern(\XSeq, \Result)$, where every~$X_i$
is an over integer interval domain~$\Domain$.
%
For every feature/aggregator pair~$\Tuple{f,g}$ our aim is to develop formulae that are
parametrised by regular expression $\pattern$ and give the sharp upper
(respesctively lower) bound on the value of $\Result$.
%
An upper (resp.\ lower) bound is sharp if it equals to  the value of
$\Result$ on at least one  time series.
%
The developed bounds are valids regardless of the domain choice but
their sharpness is guaranteed only on condition that every $X_i$ is
over the same integer interval domain.

% For each regular expression, there exists a necessary condition, based
% on the domains and number of the~$X_i$, for it to occur at least once
% within the signature.

% \begin{example}
%   \label{ex:nec:cond:inflexion}
%   An $\InflexionPatternName$-pattern, called an \emph{inflexion},
%   within a time series $X = \sequence{X_1,\dots,X_\seqlength}$
%   corresponds, except for its first and last elements, to a maximal
%   occurrence of the regular expression
%   $\InflexionPatternName = \reg{(<(<|=)*>)|(>(>|=)*<)}$ in the
%   signature of~$X$.
%   % 
%   The necessary condition for having at least one inflexion in $X$ is
%   $\DomainMax > \DomainMin \land \seqlength \geq 3$, where
%   $\Domain$ is the smallest interval containing the
%   union of the domains of the~$X_i$. \figref{fig:inflexion_occurrence}
%   gives an example of inflexion.  \qed
% \end{example}

% \input{inflexion-time-series-figure.tex}  

In \secref{sec:methodology}, we \new{recall} a systematic methodology
\new{introduced in~\cite{CP16}} for
deriving sharp bounds on~$\Result$ for any time-series constraint
$\Constraint{g\_f}\_\pattern(\Tuple{X_1, \dots, X_\seqlength}, \Result)$, under the
assumptions that all the~$X_i$ have the same interval domain and,
without loss of generality, that the underlying necessary condition
holds.
%
\new{We also give the structure of the following sections.}

% Do NOT erase the following lines:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "bounds.tex"
%%% End:


==> shift.tex <==
\subsection{Shift}
\label{sec:shift}

This sections introduces the notion of shift of a regular expression,
which is used for deriving the sharp bounds when the feature is
in~$\Curly{\MaxFeature, \MinFeature}$ and the aggregator is~$\SumAggr$.
\todotext{To complete!}


\todotext{Not gonna be used for the 1st journal paper!}
\begin{definition}
\label{def:shift-one-word}
\IntroDom{\pattern}{\Domain}.
%
\DefinitionArg{shift}{a word~$\wordv$ in~$\Language{\pattern}$}{\DomainMin,
  \DomainMax}{\CharAllSigma{\Shift}{\pattern}{\DomainMin,
    \DomainMax}{\wordv}}{\SetRegExpressions \times \Integers \times \Integers
\times \AllWords}{\Naturals}{}
%
It is defined by the following formula~$\CharAllSigma{\Shift}{\pattern}{\DomainMin,
    \DomainMax}{\wordv} = \min \limits_{\TimeSeries \in
    \CharAll{\SupportSet}{\pattern}{\DomainMin,
  \DomainMax}{\wordv}} \min \limits_{x \in \TimeSeries_\word} (\max(\TimeSeries) -
x)$, where~$\max(\TimeSeries)$ is the maximal value of a
time series~$\TimeSeries$ and~$\TimeSeries_\word$ is the~$\pattern$-pattern
of~$\TimeSeries$ corresponding to the occurrence of~$\word$ in the
signature of~$\TimeSeries$.

\nomenclature[1]{${\CharAll{\Shift}{\pattern}{\DomainMin,
      \DomainMax}{\wordv, \word}}$}{the \emph{shift} of a
  subword~$\word$ within a word~$\wordv$ in~$\Language{\pattern}$
  wrt~$\Tuple{\DomainMin,
    \DomainMax}$ (see~\defref{def:shift-two-words})}
\end{definition}







% Do NOT erase the following lines:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "bounds.tex"
%%% End:
